Separability and Non-Determinizability of WSTS

We study the languages recognized by well-structured transition systems (WSTS) with upward and downward compatibility. Our first result shows that every pair of disjoint WSTS languages is regularly separable: there is a regular language containing one of them while being disjoint from the other. As a consequence, if a language as well as its complement are both recognized by WSTS, then they are necessarily regular. Our second result shows that the languages recognized by deterministic WSTS form a strict subclass of the languages recognized by all WSTS: we give a non-deterministic WSTS language that we prove cannot be recognized by a deterministic WSTS. The proof relies on a novel characterization of the languages accepted by deterministic WSTS.

==> content/cts_unused.tex <==
%For this reason, we take this section to develop a deterministic model that is equivalent to WSTS.
%

%
% and respects these requirements.
%
%Working with CTS rather than determinized WSTS leads to a cleaner development (we can avoid products and downward-closed sets) and allows us to highlight key arguments.
%
%The plan is to invoke the proof principle for regular separability, Theorem~\ref{thm:core}, and show that the product system has a finitely represented inductive invariant.
%
%As we discussed, the principle holds for general ULTS but needs one of them deterministic.
%
%Therefore, 


Our first step is to determinize the given WSTS.
%Determinizing a WSTS will yield an ULTS, but may ruin the WQO property.
%
%We show that the set of states of the resulting ULTS still has a rich structure: it is a powerset lattice in which every infinite sequence contains a subsequence that converges in a natural sense.
%
%We call such ULTS converging transition systems (CTS).
%
%


==> content/dwsts_unused.tex <==

%
%The details are in the full version~\cite{keskinmeyer2023sep}.
\begin{comment}
%
\begin{proof}
Let $\anults=(\states, \leq, \initstates, \analph, \transitions, \finalstates)$ be a deterministic \ults.
That $\complementof{\anults}$ accepts the complement language is due to Rabin and Scott.
%
To see that $\geq$ is a simulation, consider $\astate_1,\astatep_1, \astatep_2\in\states$, and $\aletter\in\analph$ with $\astate_1\leq\astatep_1$ and $\astatep_2\in\transitions(\astatep_1, \aletter)$.
By determinism, there is $\astate_2\in \transitions(\astate_1, \aletter)$.
As $\leq$ is a simulation, we obtain $\astatep_3\in \transitions(\astatep_1, \aletter)$ with $\astate_2\leq \astatep_3$.
By determinism, $\astatep_3=\astatep_2$ has to hold.
\end{proof}
\end{comment}
\begin{comment}
 By upward compatbility, we have
%
Upward-compatibility and determinicity force the unique transition $(\astate, \aletter, \astate')\in\transitions$ to exist where $\astatep'\leq\astate'$ for $(\astatep, \aletter, \astatep')\in\transitions$.
%
Since $\finalstates$ is upward-closed, $\complementof{\finalstates}$ is downward-closed.
%
So $(\states, \leq, \initstates, \analph, \transitions, \complementof{\finalstates})$ is a valid DLTS.
%
Thanks to determinicity it accepts $\complementof{\langof{\anults}}$.
%
We gather both observations in the lemma below.


Here $=_{rev}$ refers to reverse-equality and $=_{cmp}$ refers to compliment-equality.
%
We say that the language class $\langof{X}$ \emph{reverse-includes} the language class $\langof{Y}$, denoted $\langof{X}\subseteq_{rev}\langof{Y}$, if $\reverseof{\alang}\in\langof{Y}$ for all $\alang\in\langof{X}$.
%
We write $\langof{X}=_{rev}\langof{Y}$ if $\langof{X}\subseteq_{rev}\langof{Y}$ and
$\langof{Y}\subseteq_{rev}\langof{X}$.
%
Compliment-equality is defined similarly wrt. $\subseteq_{cmp}$.
%
We say $\langof{X}\subseteq_{cmp}\langof{Y}$ if for all $\alang\in\langof{X}$, $\complimentof{\alang}\in\langof{Y}$ holds.
\end{comment}


\begin{comment}
\begin{proof}
Consider $\alang_1, \alang_2\in\langof{\downwsts}$ with $\alang_1\cap\alang_2=\emptyset$.
By Lemma~\ref{Lemma:Reversal}, $\reverseof{\alang_1}$ and $\reverseof{\alang_2}$ are languages of upward-compatible \wsts.
They are still disjoint.
We can thus apply Theorem~\ref{Theorem:RegSep} and get a regular language $\areg$ that separates $\reverseof{\alang_1}$ and~$\reverseof{\alang_2}$.
The regular languages are closed under reversal, and so $\reverseof{\areg}$ separates $\alang_1$ and $\alang_2$.
\end{proof}
\end{comment}
% (regular separability for upward-compatible WSTS), the closure of regular languages under reversal, and Lemma~\ref{Lemma:DWSTSLanguages}, we get the result we seek.

==> content/ideal_separability.tex <==
\section{A Specialized Invariant Construction for \dwsts}\label{Section:SimpleRegSep}
In Sections \ref{Section:CTS} and \ref{Section:FullRegSep}, we show Theorem~\ref{Theorem:RegSep}.
%
The construction extends an arbitrary invariant into a finitely represented one, and works with convergence arguments.
%
However, if we restrict Theorem~\ref{Theorem:RegSep} into Theorem~\ref{Theorem:RegSepLimited} below, a more direct construction becomes possible.
%
\begin{thm}\label{Theorem:RegSepLimited}
    For $\alang_1\in\langof{\upwsts}$ and $\alang_{2}\in\langof{\dwsts}$, we have $\alang_1\regsep\alang_2$ if and only if $\alang_1\cap\alang_2=\emptyset$.
\end{thm}

In the following, we give an invariant construction for Theorem~\ref{Theorem:RegSepLimited} that (i) merely decomposes an arbitrary invariant (ii) works with better known concepts.
%
The key to our construction is the notion of ideal completions \cite{InfBranching14,FG09}.
%
We show that any invariant for a \WSTS yields a
finitely-represented invariant for the corresponding ideal completion.
%
Theorem~\ref{Theorem:RegSepLimited} follows from this.

An \emph{ideal} in a  \wqo $(X, \leq)$ is a non-empty downward-closed subset $Z\subseteq X$ which is directed:
For every $z, z'\in Z$ there is a $z'' \in Z$ with $z  \leq z''$ and $z' \leq z''$.
Every downward-closed set decomposes into finitely many ideals.
In fact, the finite antichain property is sufficient and necessary for this.

\begin{lem}[\cite{KP92,FG09,LS15}]
\label{lem:idec}
    In a \wqo, every downward-closed set is a finite union of ideals.
\end{lem}
%
\noindent
We use $\idec{X}{Z}$ to denote the set of inclusion-maximal ideals in $Z$.
By the above lemma, $\idec{X}{Z}$ is always finite and
%
\begin{align}
\label{eq:union}
    Z = \bigcup \idec{X}{Z}\ .
\end{align}
%
\noindent
We will also make use of the fact that ideals are irreducible in the following sense.

\begin{lem}[\cite{KP92,FG09,LS15}]
\label{lem:idealsirred}
    Let $(X, \leq)$ be a \wqo.
    If $Z \subseteq X$ is downward-closed and $I \subseteq Z$ is an ideal, then
    $I \subseteq J$ for some $J \in \idec{X}{Z}$.
\end{lem}

The \emph{ideal completion} $(\idcompl{X}, \subseteq)$ of $(X, \leq)$ has as elements all ideals
in $X$.
%
The order is inclusion.
%
The ideal completion $\idcompl{X}$ can be seen as extension of $X$; indeed, every element $x\in X$ is represented
by $\downclosure{\{x\}} \in \idcompl{X}$, and inclusion among such representations
coincides with the original quasi order~$\leq$.
%
Later, we will also need general ideals that may not be the downward closure of a single element.

%Intuitively, the goal is to invoke Lemma~\ref{lem:idec}.
In \cite{FG09,InfBranching14}, the notion has been lifted to \WSTS\ $\anults=(\states, \leq, \initstates, \analph, \transitions, \finalstates)$.
%
The ideal completion of $\anults$ is the \ULTS $\idcompl{\anults}$, where the given $\wqo$ is replaced by its ideal completion.
%
%So configurations of $\idcompl{W}$ are ideals.
The initial configurations are the ideals in the decomposition of $\downclosure{I}$.
%
The transition relation is defined similarly, by decomposing $\downclosure{\succe{\anults}{X}{a}}$, with $X$ an ideal.
%
The final configurations are the ideals that intersect $F$.

\begin{defi}[\cite{FG09,InfBranching14}]
    For a \UWSTS $\anults = (\states, \leq, \initstates, \analph, \transitions, \finalstates)$, we define its \emph{ideal completion}
    $\idcompl{\anults} = (\idcompl{\states}, \subseteq, \idcompl{\initstates}, \analph, \idcompl{\transitions}, \idcompl{\finalstates})$, where
    $(\idcompl{\states}, \subseteq)$ is the ideal completion of $(\idcompl{\states}, \leq)$.
    The transition relation of $\idcompl{\anults}$ is defined by
    \(
        \idcompl{\transitions}(X, a) \ = \ \idec{S}{\downclosure{\succe{\W}{X}{a}}}\ ,
        %\succe{\idcompl{\W}}{X}{a}
    \)
    %the initial configurations
    $\idcompl{\initstates} = \idec{S}{\downclosure{I}}$, and % contains ideals in the ideal decomposition of $\downclosure{I}$,
    %the final configurations
    $\idcompl{\finalstates} = \setof{X\in\idcompl{\states}}{X\cap F \neq \emptyset}$. % are those ideals which contain some final configuration of $\W$,
    %and the transition relation is defined essentially as the downward closure of the direct image:
\end{defi}
%
\noindent
Using upward compatibility in $\anults$, language equivalence holds and determinism is preserved.

\begin{lem}
\label{lem:idcompl}
  The ideal completion $\idcompl{\anults}$ of a \UWSTS $\anults$ is a \ULTS.
  We have $\langof{\idcompl{\anults}}=\langof{\anults}$.
  If $\anults$ is deterministic, then so is $\idcompl{\anults}$.
\end{lem}
%
\noindent
As a matter of fact, $\idcompl{\anults}$ is even finitely branching, but we do not need this property.

The purpose of using ideal completions is to make it easier to find inductive invariants that are finitely represented.
%The argument is as follows.
Assume the given \UWSTS $\anults$ has an inductive invariant $X$, not necessarily finitely represented.
By definition, $X$ is downward-closed.
Thus, by Lemma~\ref{lem:idec}, $X$ is a \emph{finite} union of ideals.
These ideals are configurations of the ideal completion $\idcompl{\anults}$.
To turn $\idec{\states}{X}$ into an inductive invariant, it remains to take the downward closure of the set.
As the order among ideals is inclusion, this does not add configurations.
In short, an inductive invariant for $\anults$ induces a finitely-represented inductive invariant for $\idcompl{\anults}$.

\begin{prop}
\label{prop:inducedinvariant}
    If $X \subseteq S$ is an inductive invariant of $\anults$,
    $\downclosure{\idec{\states}{X}}$ is a finitely-represented inductive invariant of $\idcompl{\anults}$.
\end{prop}
%
\begin{proof}
    %[Proof of Proposition~\ref{prop:inducedinvariant}]
    Define $\sepstates = \idec{\states}{X}$.
    %
    Since $\sepstates$ contains all ideals $Y \subseteq X$ that are maximal wrt.~inclusion, $\downclosure{\sepstates}$ contains all ideals $Y \subseteq X$.
    We observe that
    \[
    X \stackrel{\eqref{eq:union}}{=} \bigcup \sepstates = \bigcup \downclosure{\sepstates}
    \ .
    \]
    By Lemma~\ref{lem:idec}, $\sepstates$ is finite and thus $\downclosure{Q}$ is finitely-represented.
    It remains to check that $\downclosure{\sepstates}$ satisfies the Properties~\eqref{eq:iiI}, \eqref{eq:iiF}, and~\eqref{eq:iiSucc}.

%    We need to show that any maximal ideal contained in $\downclosure{I}$ belongs to $\downclosure{Q}$.
    To show Property~\eqref{eq:iiI}, we need to prove $\idec{\states}{\downclosure{\initstates}} \subseteq \downclosure{\sepstates}$.
    %
    We have $I \subseteq X$ by Property~\eqref{eq:iiI}, and since $X$ is downward-closed, we obtain $\downclosure{I} \subseteq X$.
    Consequently, any ideal that is a subset of $\downclosure{I}$ is also a subset of $X$, and $\downclosure{Q}$ contains all such ideals.
    For Property~\eqref{eq:iiF}, assume towards a contradiction that $\downclosure{Q}$ contains an ideal $Y$ that is final in~$\idcompl{\anults}$.
    By definition, this means $Y$ contains a final configuration.
    Since $Y \subseteq X$, we obtain a contradiction to $X \cap F = \emptyset$, Property~\eqref{eq:iiF}.
%
    To check the inclusion $\succe{\idcompl{\anults}}{\downclosure{\sepstates}}{a} \subseteq \downclosure{\sepstates}$, we pick an ideal $Y \in \downclosure{\sepstates}$ and show $\succe{\idcompl{\anults}}{Y}{a} \subseteq \downclosure{\sepstates}$.
    %
    Recall the definition $\succe{\idcompl{\anults}}{Y}{a} = \idec{\states}{\downclosure{\succe{\anults}{Y}{a}}}$.
    Thus, any element of $\succe{\idcompl{\anults}}{Y}{a}$ is an ideal that is a subset of $\downclosure{\succe{\anults}{Y}{a}}$.
%
    We have $\succe{\anults}{X}{a} \subseteq X$ by Property~\eqref{eq:iiSucc}.
    This implies $\succe{\anults}{Y}{a} \subseteq X$ as $Y \subseteq X$, and even \mbox{$\downclosure{\succe{\anults}{Y}{a}} \subseteq X$} as $X$ is downward-closed.
    Hence, any ideal that is a subset of $\downclosure{\succe{\anults}{Y}{a}}$ is also subset of $X$, and thus an element of
    $\downclosure{\sepstates}$.
\end{proof}
%
Theorem~\ref{thm:core} expects invariants for \UWSTS of a particular shape, namely products $\anults\times \anultsp$.
%
We now show that the operation of ideal completion commutes with taking products of \UWSTS, a fact that will be key to the proof of Theorem~\ref{Theorem:RegSepLimited}.
%
We start by recalling that the ideals in a product \wqo $X\times Y$ are precisely the products of the ideals in $X$ and in $Y$.

\begin{lem}[\cite{KP92,FG09,LS15}]
\label{lem:prodideals}
    A set $Z\subseteq X\times Y$ is an ideal iff $Z = I \times J$, where $I \subseteq X$
    and $J\subseteq Y$ are ideals.
\end{lem}
%
\noindent
Lemma~\ref{lem:prodideals} yields the mentioned commutativity.

\begin{lem}
\label{lem:isoprod}
    For two \UWSTS $\anults$ and $\anultsp$,
%    the weak {\UWSTS}
    $\idcompl{\anults} \times \idcompl{\anultsp}$ and $\idcompl{(\anults \times \anultsp)}$ are isomorphic.
\end{lem}
%
\noindent
We are now prepared to apply Theorem~\ref{thm:core} once more to establish our second main result.

\begin{proof}[Proof of Theorem~\ref{Theorem:RegSepLimited}]
    Let $\W = (\states_{\W}, \leq_{\W}, \initstates_{\W}, \analph, \transitions_{\W}, \finalstates_{\W})$ be a \UWSTS for $\W\in\set{\anults, \anultsp}$, let $\langof{\anults}\cap\langof{\anultsp}=\emptyset$, and further let $\anultsp$ be deterministic.

    We would like to construct a finitely-represented inductive invariant in the synchronized product of the ideal completions $\idcompl{\anults} \times \idcompl{\anultsp}$ and then apply Theorem~\ref{thm:core}.
    %
    Indeed, by Lemma~\ref{lem:idcompl} we know that the ideal completions are disjoint \ULTSes, and that the latter one is still deterministic, so they satisfy the assumptions.

    Relying on Lemma~\ref{lem:isoprod} we prefer to show the existence of a finitely-represented inductive invariant in
    \(
        \idcompl{(\anults\times \anultsp)}.
    \)
    Using Proposition~\ref{prop:inducedinvariant}, it is sufficient to find any inductive invariant in $\anults\times \anultsp$, it does not have to be finitely-represented.
    %
    We know that such an inductive invariant exists by Lemma~\ref{Lemma:Invariants}, since we assume  $\langof{\anults\times \anultsp} = \langof{\anults} \cap \langof{\anultsp} = \emptyset$.
\end{proof}


==> content/separability_unused.tex <==

As we mentioned in the beginning of the section, we intend to use Theorem~\ref{thm:core} to show separability results for WSTS languages.
%
Thanks to this result, the proof of our separability theorem takes the form of invariant construction.
%
We intend to search for finitely represented invariants and use Theorem~\ref{thm:core} to convert them into separators.
%
Fortunately, we will always have the guarantee of an inductive invariant (not necessarily finitely represented).
%
This is because inductive invariants are complete for proving emptiness, like inductive invariants for programs are (relatively) complete for proving safety~\cite{Cook1978}.

\begin{lem}
\label{Lemma:Invariants}
    Consider \ULTS $U$.
    Then $\langof{U}=\emptyset$ iff there is an inductive invariant for~$U$.
\end{lem}
\noindent

To see that every inductive invariant shows language emptiness, consider the definition of the inductive invariant.
%
Let $X$ be an inductive invariant for $U$.
%
By~\eqref{eq:iiI} and~\eqref{eq:iiSucc}, the invariant has to contain the whole reachability set.
%
By~\eqref{eq:iiF} and~\eqref{eq:iiSucc}, it has to be disjoint from the predecessors of the final configurations:
%
\begin{align*}
%    \label{eq:iiReach}
    &\reachall{\W} \subseteq X
    \ ,
    &
%    \label{eq:iiReveach}
    &\revreachall{\W} \cap X = \emptyset
    \ .
\end{align*}
%
Combined, these results show language emptiness.

For completeness in the context of \ULTS, observe that $X = \downclosure{\reachall{\W}}$ is an inductive invariant if the language is empty.
%
It is the least one wrt.~inclusion.
%
There is also a greatest inductive invariant, namely the complement of $\revreachall{\W}$.
%
Note that, due to upward compatibility, $\revreachall{\W}$ is always upward-closed.

%The advantage of inductive invariants over these two sets is the possibility of approximation.
%Also invariants larger than the reachability set and smaller than the predecessors of the final states will prove language emptiness.
Other invariants may have the advantage of being easier to represent.
We will be particularly interested in invariants that are finitely represented in the sense that they form the downward closure of a finite set.



%\begin{thm}
%\label{thm:core}
%    Let $\W$ and $\W'$ be disjoint \ULTSes, one of them deterministic, such that $\W \times \W'$ admits a finitely-represented inductive invariant $\downclosure{Q}$.
%    Then $\W$ and $\W'$ are regular separable by the language of a finite automaton with states $Q$.
%\end{thm}
%
\noindent

%
Unfortunately, Theorem~\ref{thm:core} introduces a conflict between our goal, and our preferred methods.
%
On the one hand, we want to show a result that concerns all \WSTSes, while on the other hand, we want to make use of the \WSTS structure while searching for the invariant.
%
The source of the incompatiblility is that we need one of the ULTS to be deterministic if we want to apply Theorem~\ref{thm:core}.
%
However, it is well known that WSTS are not closed under naive determinization \cite{JANCAR1999}.\sm{Need to find a a way to fix this one...}
%
In fact, we show in Section~\ref{Section:NonDet} that determinism is a real restriction to the expressive power of WSTS.

We tackle this incompatibility by giving up our preferred method.
%
We accept that we need to search for invariants in a class of \ULTS that has less structure than \WSTS .
%
In Section~\ref{Section:FullRegSep}, we see that this suffices to find finitely represented inductive invariants and thus show Theorem~\ref{Theorem:RegSep}.
%
However, we also present an alternative approach.
%
In Section~\ref{Section:SimpleRegSep}, we prove a limited separability result that assumes one of the \WSTS to be deterministic.
%
This restriction allows us to work with well-known WQO-theoretical tools, resulting in a more direct invariant construction.
%
We extend the scope of this technique in Section~\ref{Section:NonDet} by showing that almost all widely-used WSTS models determinize.
